Knowledge Graph Augmented Large Language Models for Disease Prediction

Electronic health records (EHRs) enable strong clinical prediction, but explanations are often coarse and hard to use for patient-level decisions. We propose a knowledge graph (KG)-guided chain-of-thought (CoT) framework for visit-level disease prediction on MIMIC-III. We map ICD-9 codes to PrimeKG, mine disease-relevant nodes and paths, and use these paths to scaffold temporally consistent CoT rationales, retaining only samples whose conclusions match observed outcomes. We fine-tune lightweight instruction-tuned LLMs (LLaMA-3.1-Instruct-8B and Gemma-7B) on two small cohorts (400 and 1,000 index visits) across ten PrimeKG-mapped diseases. Our models outperform strong classical baselines, reaching AUROC 0.66-0.70 and macro-AUPR 0.40-0.47. Without additional training, the models transfer zero-shot to the CRADLE cohort, improving accuracy from 0.40-0.51 to 0.72-0.77. In a blinded clinician study, KG-guided CoT rationales are consistently preferred for clarity, relevance, and correctness. Code is available at: https://github.com/JonathanWry/KG-guided-LLM-pipeline

==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related-works}
Predictive modeling with EHR data has been studied extensively for outcomes such as mortality, readmission, and disease onset, with MIMIC-III serving as a widely used benchmark cohort.\cite{johnson2016mimic,goldstein2017practical} Classical models such as logistic regression and tree-based ensembles remain popular due to their robustness, interpretability at the global level, and ease of deployment in clinical systems.\cite{goldstein2017practical} In addition to classical models, neural architectures including recurrent networks and attention-based models have been explored for modeling temporal dynamics and co-occurrence patterns in EHR data.\cite{ruan2019representation}
Despite these advances in predictive performance, most EHR models provide only coarse, post hoc interpretability via feature importance or attention weights, which offer limited support for patient-specific, clinician-facing reasoning about why a particular outcome is likely.

In parallel, Chain-of-Thought (CoT) prompting has emerged as an effective strategy for eliciting structured, step-by-step reasoning in large language models, with substantial gains reported on mathematics, scientific question answering, and broad reasoning benchmarks.\cite{huang202202cot,xie2024reasoning} Recent work on data-efficient reasoning further highlights the importance of high-quality CoT supervision and careful scaling strategies.\cite{muennighoff2025,ye2025} However, the application of CoT in medicine remains underdeveloped: clinically validated reasoning datasets are scarce, and unconstrained CoT reasoning can introduce hallucinated or medically incorrect intermediate steps, which is particularly problematic in high-stakes clinical decision making.\cite{liu2025ragreview}

These limitations have motivated efforts to constrain or ground LLM reasoning using external knowledge sources to improve factual reliability. Biomedical knowledge graphs (KGs) such as PrimeKG integrate curated relationships among diseases, phenotypes, drugs, and genes, and have been leveraged to enhance factual grounding in medical question answering and decision-support systems.\cite{chandak2023primekg,liu2025ragreview} Recent knowledge graph aided LLM approaches suggest that conditioning LLMs on KG-derived information can improve the logical consistency and factual grounding of generated explanations.\cite{wang2025superrelations} 

Our work connects these lines of research by integrating biomedical KG structure directly into the CoT generation process for visit-level disease prediction on structured EHR data. Instead of relying on unconstrained free-form explanations, we construct disease-specific reasoning paths in PrimeKG\cite{chandak2023primekg}, use them as scaffolds to guide CoT generation, and retain only those reasoning traces whose conclusions match observed patient outcomes. This KG-anchored supervision enables data-efficient prognostic learning and supports interpretable, patient-level reasoning without requiring KG access at inference time.
